Cooperative Starting Movement Detection of Cyclists Using Convolutional Neural Networks and a Boosted Stacking Ensemble

In future, vehicles and other traffic participants will be interconnected and equipped with various types of sensors, allowing for cooperation on different levels, such as situation prediction or intention detection. In this article we present a cooperative approach for starting movement detection of cyclists using a boosted stacking ensemble approach realizing feature- and decision level cooperation. We introduce a novel method based on a 3D Convolutional Neural Network (CNN) to detect starting motions on image sequences by learning spatio-temporal features. The CNN is complemented by a smart device based starting movement detection originating from smart devices carried by the cyclist. Both model outputs are combined in a stacking ensemble approach using an extreme gradient boosting classifier resulting in a fast and yet robust cooperative starting movement detector. We evaluate our cooperative approach on real-world data originating from experiments with 49 test subjects consisting of 84 starting motions.

==> cv.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{stefan}}]{Stefan Zernetsch}
received the B.Eng. and the M.Eng. degree in Electrical Engineering and Information Technology from the University of Applied Sciences Aschaffenburg, Germany, in 2012 and 2014, respectively. Currently, he is working on his PhD thesis in cooperation with the Faculty of Electrical Engineering and Computer Science of the University of Kassel, Germany. His Research interests include cooperative sensor networks, sensor data fusion, multiple view geometry, pattern recognition and short-term behaviour recognition of traffic participants.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{kdoll}}]{Konrad Doll}
received the Diploma (Dipl.-Ing.) degree and the Dr.-Ing. degree in Electrical Engineering and Information Technology from the Technical University of Munich, Germany, in 1989 and 1994, respectively. In 1994 he joined the Semiconductor Products Sector of Motorola, Inc. In 1997 he was appointed to professor at the University of Applied Sciences Aschaffenburg in the field of computer science and digital systems design. Since 2016 he is a research Professor for cooperative automated traffic systems. His research interests include intelligent systems, their real-time implementations on platforms like CPU, GPUs and FPGAs and their applications in advanced driver assistance systems and automated driving. Konrad Doll is member of the IEEE.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bsick}}]{Bernhard Sick}
received the diploma, the Ph.D. degree, and the "Habilitation" degree, all in computer science, from the University of Passau, Germany, in 1992, 1999, and 2004, respectively. Currently, he is full Professor for intelligent embedded systems at the Faculty for Electrical Engineering and Computer Science of the University of Kassel, Germany. There, he is conducting research in the areas autonomic and organic computing and technical data analytics with applications in biometrics, intrusion detection, energy management, automotive engineering, and others. He authored more than 90 peer-reviewed publications in these areas.\\
Dr. Sick is associate editor of the IEEE TRANSACTIONS ON CYBERNETICS. He holds one patent and received several thesis, best paper, teaching, and inventor awards. He is a member of IEEE (Systems, Man, and Cybernetics Society, Computer Society, and Computational Intelligence Society) and GI (Gesellschaft fuer Informatik).
\end{IEEEbiography}


==> sections/method_overall.tex <==
\subsection{Cooperative Trajectory Forecast}
\label{sec_method_overall}




==> sections/method_prediction.tex <==
\subsection{Trajectory Forecast}
%\label{sec_method_cv}




==> sections/results_prediction.tex <==
\subsection{Trajectory Forecast}





==> sections/results_trajectories.tex <==
\subsection{Data Acquisition}
\label{sec_data_acquisition}


\subsection{Trajectory Extraction}
\label{sec_results_trajectory_generation}

%The starting point is defined as the point in time at which the 
%rear wheel starts to move and a subsequent forward motion is recognizable. The starting points are labeled by human operators. 

